SizeFlags: Reducing Size and Fit Related Returns in Fashion E-Commerce

E-commerce is growing at an unprecedented rate and the fashion industry has recently witnessed a noticeable shift in customers' order behaviour towards stronger online shopping. However, fashion articles ordered online do not always find their way to a customer's wardrobe. In fact, a large share of them end up being returned. Finding clothes that fit online is very challenging and accounts for one of the main drivers of increased return rates in fashion e-commerce. Size and fit related returns severely impact 1. the customers experience and their dissatisfaction with online shopping, 2. the environment through an increased carbon footprint, and 3. the profitability of online fashion platforms. Due to poor fit, customers often end up returning articles that they like but do not fit them, which they have to re-order in a different size. To tackle this issue we introduce SizeFlags, a probabilistic Bayesian model based on weakly annotated large-scale data from customers. Leveraging the advantages of the Bayesian framework, we extend our model to successfully integrate rich priors from human experts feedback and computer vision intelligence. Through extensive experimentation, large-scale A/B testing and continuous evaluation of the model in production, we demonstrate the strong impact of the proposed approach in robustly reducing size-related returns in online fashion over 14 countries.

==> sections/extentions.tex <==
The fully Bayesian model discussed in~\autoref{sec:full-model} requires additional information to be integrated as prior knowledge within the algorithm. In this section we present two extensions which leverage two different sources of expert knowledge: In~\autoref{sec:human-feedback} we explain how to integrate feedback from human models, and in~\autoref{sec:sizenet} we show how to use previous work on extracting sizing information from article images~\cite{sizenet} to incorporate prior information about articles even before any order is observed. Finally, in~\autoref{sec:threshold-opt} we introduce a third extension by studying closely both conditions in ~\autoref{eq:combined-conditions-flag-posterior} and trying to optimize the threshold $\theta$ to enable raising flags with less article orders and returns. The combination of these three extensions allows us to tackle the cold-start problem on a large-scale and in a robust and efficient manner, thus constitute our final SizeFlags algorithm. 

\subsection{Human expert feedback}\label{sec:human-feedback}
To incorporate expert knowledge from human feedback we ask human fashion models with relatively standard body sizes to try on articles before they are online on the platform and give us size and fit feedback. For the purpose of this paper, we constrain the nature of the feedback to be one of \{``certain size issue", ``potential size issue", ``good fit"\}. Multiple human models can fit the same article and based on the aggregated feedback we define article-specific prior parameters $(\alpha, \beta)$. If the aggregated feedback points strongly in the direction of a size issue, we chose values which strongly favor high return rates, if the aggregated feedback is more uncertain we favor more mildly high return rates, and if the aggregated feedback points towards a good fit we favor low return rates. 

\subsection{Size and fit visual cues}
\label{sec:sizenet}
Using the full Bayesian model presented in ~\autoref{sec:full-model} with human feedback does help alleviate the cold-start problem but it does not totally suppress the issue. In fact, a well trained group of human models can only fit a very limited part of the ever changing online assortment every week (less than $1\%$), which means only a few articles have specific parameter values $(\alpha, \beta)$ for the prior distribution, whereas for all the remaining articles, default - and thus uninformative - values are used (e.g. values such that the prior favors return rates around $\pi$), thereby causing the cold-start problem to persist. For our second extension, we thus propose to use size and fit visual cues - which are easier to obtain - in our full Bayesian model. Although the literature is very rich on computer vision techniques for various fashion problems, there are only few works considering fashion images for the size and fit problem (see \cite{Hsiao2020, sizenet} and references therein). We use our fully Bayesian model by incorporating sizing information extracted from article images using SizeNet~\cite{sizenet}.

More specifically, the output of a SizeNet~\cite{sizenet} model is a size issue probability which we propose to convert into prior values \textcolor{darkgreen}{$(\alpha, \beta)$} of the Beta distribution. This extension enables us to incorporate article size and fit information from visual cues which, unlike human expert feedback, can be provided at scale. In other words. whenever human feedback is available for an article, we use it directly to shape the prior Beta distribution; when such information is unavailable, which is the case for most articles, we employ the SizeNet~\cite{sizenet} model instead to shape the prior Beta distribution. For more details about the SizeNet model~\cite{sizenet}, we refer the reader to Section 2 of the supplementary material. In our setting, the teacher model used to produce class labels (size issue or not) to train the student network~\cite{bracher2016fashion} is the baseline binomial model described in~\autoref{subsec:binomial}.


%SizeNet~\cite{sizenet} introduces a teacher-student framework which learns size issue from article images. Let us denote image and class pairs $x_i \in X$ and $y_i \in Y$ from a training set $S= \{(x_i,y_i), i=1..n\}$ with $y_i$ being the class label (size issue or not) produced by a teacher model, which, in our case, is produced by the baseline binomial model described in~\autoref{subsec:binomial}. A sample weight $w_i$ is then defined as:  
%\begin{equation}
%        w_i = \ln{(1+s_i)}
%    \label{eq:sample_weight}
%\end{equation} 
%The student model consists of 1) a backbone network~\cite{bracher2016fashion} $\phi: X \rightarrow{} \tilde X$ used as a bottleneck image features extractor; and 2) a multi-layer perceptron (MLP) on top that learns a function $f: \tilde X \rightarrow{} Y$ using the following objective:
%\begin{equation}
%         \min_\theta \sum_{i=1}^{n} w_i L(y_i,f(\phi(x_i);\theta))
%    \label{eq:sizenet_objective}
%\end{equation} 
%where $L$ is the binary cross-entropy loss function, $y_i$ is the teacher label, $f(\phi(x_i))$ is the predicted label, and $w_i$ is the sample confidence score from~\autoref{eq:sample_weight}. 

%Similarly to human expert feedback (\autoref{sec:human-feedback}), we translate the obtained image-based size issue predictions into parameter values \textcolor{darkgreen}{$(\alpha, \beta)$} for the prior distribution, favoring different regions of size-related return rates based on the size issue probability obtained by SizeNet student model~\cite{sizenet}.


%\subsection{Threshold optimization}\label{sec:threshold-opt}

%With a very conservative threshold $\theta$, in the lifetime of an article on the platform, the second condition of ~\autoref{eq:combined-conditions-flag-posterior} $k/n > \pi + \sigma$ will almost always be verified much earlier before the first one. An analytical study has showed that often, the empirical return rate of an article $k/n$ stabilizes around its true expected value fairly rapidly. Numerous days or weeks can pass between the time the condition $k/n > \pi + \sigma$ is stably verified and the time when the second condition $- \log p(\pi | k,n; \, \alpha, \beta) > \theta$ gets verified (if it is ever verified). While setting a conservative value for $\theta$ makes the algorithm more robust to noise in the data and increases the confidence in the flags raised ($p(\pi | k,n;\, \alpha, \beta)$ has to be really low for a size issue flag to be raised), setting its value too high hinders the algorithm's performance as too high numbers of article orders and returns ($n$ and $k$) are necessary to raise a size issue flag, therefore counteracting the main goal of the algorithm. 

%With $\theta_{\text{max}}:=15$ as a  conservative baseline threshold, which corresponds to an upper bound on the binomial likelihood of $3.10^{-7}$, we describe now an optimization problem that delivers an optimal value $\theta^\star$ in order to obtain almost the same size issue flags as before, only much faster. We select such a $\theta^\star$ according to the following optimization problem:
%\begin{align} \label{eq:threshold_optimization}
%    &\theta^\star = \argmin_{\theta \in (0, \, \theta_{\text{max}}]} \theta \ \ \text{ subject to } \ \ \frac{N(\theta)-S(\theta)}{N(\theta)} \leq \varepsilon_1, \\ \nonumber
%    &\frac{N(\theta)-N(\theta_{\max})}{N(\theta_{\max})} \leq \varepsilon_2, \ \ \ \frac{N(\theta)-S(\theta)}{N(\theta_{\max})-S(\theta_{\max})} \leq \varepsilon_3.
%\end{align}

%We denote by $N(\theta)$ the number of articles flagged by the algorithm with parameter $\theta$ and by $S(\theta)$ (the stability) the number of flags raised whose value does not change across the time period considered. Thus, the difference $N(\theta)-S(\theta)$ can be seen as the number of unstable flags. 

%The second constraint of (\ref{eq:threshold_optimization}) restricts the number of additional flags compared to the baseline ($N(\theta)$ is increasing when $\theta$ decreases). Last but not least, the third constraint translates that the ratio of unstable flags with parameter $\theta$ compared to the same ratio with the baseline $\theta=\theta_{\text{max}}$ must be restricted by a parameter $\varepsilon_3$. The parameters $\varepsilon_i$ are values set to ensure the flags raised using a threshold $\theta$ are similar in number and quality to those raised by baseline. Due to the monotony behavior of the constraints, $\varepsilon_1, \varepsilon_2\in(0,1)$ and $\varepsilon_3\geq 1$.


